The MineRL 2019 Competition on Sample Efficient Reinforcement Learning using Human Priors

Though deep reinforcement learning has led to breakthroughs in many difficult domains, these successes have required an ever-increasing number of samples. As state-of-the-art reinforcement learning (RL) systems require an exponentially increasing number of samples, their development is restricted to a continually shrinking segment of the AI community. Likewise, many of these systems cannot be applied to real-world problems, where environment samples are expensive. Resolution of these limitations requires new, sample-efficient methods. To facilitate research in this direction, we introduce the MineRL Competition on Sample Efficient Reinforcement Learning using Human Priors. The primary goal of the competition is to foster the development of algorithms which can efficiently leverage human demonstrations to drastically reduce the number of samples needed to solve complex, hierarchical, and sparse environments. To that end, we introduce: (1) the Minecraft ObtainDiamond task, a sequential decision making environment requiring long-term planning, hierarchical control, and efficient exploration methods; and (2) the MineRL-v0 dataset, a large-scale collection of over 60 million state-action pairs of human demonstrations that can be resimulated into embodied trajectories with arbitrary modifications to game state and visuals. Participants will compete to develop systems which solve the ObtainDiamond task with a limited number of samples from the environment simulator, Malmo. The competition is structured into two rounds in which competitors are provided several paired versions of the dataset and environment with different game textures. At the end of each round, competitors will submit containerized versions of their learning algorithms and they will then be trained/evaluated from scratch on a hold-out dataset-environment pair for a total of 4-days on a prespecified hardware platform.

==> sections/competititon_description/domain_interest.tex <==
    \newpage
    \subsubsection{Domain Interest}

    \begin{figure}
        \begin{center}
            \includegraphics[width=0.9\textwidth]{./assets/item_hierarchy_final.png}
            \caption{\small A subset of the Minecraft item hierarchy (totaling 371
            unique items). Each node is a unique Minecraft item, block, or non-player character, and a directed edge between two nodes denotes that
            one is a prerequisite for another. Each item presents is own unique
            set of challenges, so coverage of the full hierarchy by one player
            takes several hundred hours.}
            \label{fig:hierarchicality}
        \end{center}
        \vspace{-19pt}
    \end{figure}

Minecraft is a compelling domain for the development of reinforcement and imitation learning based methods because of the unique challenges it presents: Minecraft is a 3D, first-person, open-world game centered around the gathering of resources and creation of structures and items. 
Notably, the procedurally generated world is composed of discrete blocks that allow modification; over the course of gameplay, players change their surroundings by gathering resources (such as wood from trees) and constructing structures (such as shelter and storage).
Since Minecraft is an embodied domain and the agent's surroundings are varied and dynamic, it presents many of the same challenges as real-world robotics domains. 
Therefore, solutions created for this competition are a step toward applying these same methods to real-world problems. 

An additional reason Minecraft is an appealing competition domain is its popularity as a video game; of all games ever released, it has the second-most total copies sold. 
Given its popularity, potential participants are more likely to be familiar with it than other domains based on video games. 
Likewise, the competition will be of greater interest due to its relationship with such a well-known game. %

Furthermore, there is existing research interest in Minecraft. 
With the development of Malmo~\cite{johnson2016malmo}, a simulator for Minecraft, the environment has garnered great research interest:
many researchers~\cite{shu2017hierarchical, tessler2017deep, oh2016control} have leveraged Minecraft's massive hierarchality and expressive power as a simulator to make great strides in language-grounded, interpretable multi-task option-extraction, hierarchical lifelong learning, and active perception. 
However, much of the existing research utilizes toy tasks in Minecraft, often restricted to 2D movement, discrete positions, or artificially confined maps unrepresentative of the intrinsic complexity that human players typically face. 
These restrictions reflect the difficulty of the domain, the challenge of coping with fully-embodied human state- and action-spaces, and the complexity exhibited in optimal human policies. 
Our competition and the release of the large-scale \minenet-v0 dataset of human demonstrations will serve to catalyze research on this domain in two ways: (1) our preliminary results indicate that through imitation learning, basic reinforcement learning approaches can finally deal directly with the full, unrestricted state- and action-space of Minecraft;  and (2) due to the difficult and crucial research challenges exhibited on the primary competition task, \texttt{ObtainDiamond}, we believe that the competition will bring work on the Minecraft domain to the fore of sample-efficient reinforcement learning research. \todo{@steph, could you please review these last two centences.}
   
   
